Complex Bounded Operators in Isabelle/HOL

We present a formalization of bounded operators on complex vector spaces in Isabelle/HOL. Our formalization contains material on complex vector spaces (normed spaces, Banach spaces, Hilbert spaces) that complements and goes beyond the developments of real vectors spaces in the Isabelle/HOL standard library. We define the type of bounded operators between complex vector spaces (cblinfun) and develop the theory of unitaries, projectors, extension of bounded linear functions (BLT theorem), adjoints, Loewner order, closed subspaces and more. For the finite-dimensional case, we provide code generation support by identifying finite-dimensional operators with matrices as formalized in the Jordan_Normal_Form AFP entry.

==> macros.tex <==
\makeatletter

\newcommand\emailaddress[1]{\href{mailto:#1}{#1}}

% \showafter{year}{month}{day}{text} evaluates to {text} starting from year/month/day
\newcommand\showafter[4]{%
  \ifnum\year>#1\relax
    #4% today.year > args.year
  \else
    \ifnum\year=#1\relax
    % today.year = args.year
      \ifnum\month>#2\relax
      % today.month > args.month
        #4%
      \else
        \ifnum\month=#2\relax
        % today.month = args.month
          \ifnum\day>#3\relax
          % today.day >= args.day
            #4%
          \else
            \ch@removeduplicatespace
          \fi
        \else
          \ch@removeduplicatespace
        \fi
      \fi
    \else
      \ch@removeduplicatespace
    \fi
  \fi}




\def\parenthesis@resizecommand@open{}
\def\parenthesis@resizecommand@close{}
\def\parenthesis@#1#2#3#4#5{%
  \global\let\parenthesis@resizecommand@open\empty
  \global\let\parenthesis@resizecommand@close\empty
  #1#3%
  {#5}%
  #2#4%
}
\DeclareRobustCommand\parenthesis[3]{%
  \expandafter\expandafter\expandafter
  \parenthesis@\expandafter\expandafter\expandafter{\expandafter\parenthesis@resizecommand@open\expandafter}\expandafter{\parenthesis@resizecommand@close}{#1}{#2}{#3}}


% #1=bigl #2=bigr #3=( #4=txt #5=) #6=txt #7=( #8=txt #9=)
\def\double@parenthesis@#1#2#3#4#5#6#7#8#9{%
  \global\let\parenthesis@resizecommand@open\empty
  \global\let\parenthesis@resizecommand@close\empty
  #1#3{#4}#2#5%
  {#6}%
  #1#7{#8}#2#9%
}

\DeclareRobustCommand\doubleParenthesis[7]{%
  \expandafter\expandafter\expandafter
  \double@parenthesis@\expandafter\expandafter\expandafter{\expandafter\parenthesis@resizecommand@open\expandafter}\expandafter{\parenthesis@resizecommand@close}{#1}{#2}{#3}{#4}{#5}{#6}{#7}}


\DeclareRobustCommand\resize@next@paren[2]{%
  \gdef\parenthesis@resizecommand@open{#1}%
  \gdef\parenthesis@resizecommand@close{#2}%
}

\newcommand\paren{\parenthesis()}
\newcommand\braces{\parenthesis\{\}}
\newcommand\brackets{\parenthesis[]}

\newcommand\pb{\resize@next@paren\bigl\bigr}
\newcommand\pbb{\resize@next@paren\biggl\biggr}
\newcommand\plr{\resize@next@paren\left\right}
\newcommand\pB{\resize@next@paren\Bigl\Bigr}

\DeclareRobustCommand\isaconst[1]{\texttt{\frenchspacing\external@render{CONST:#1}}}
\DeclareRobustCommand\isaconstpre[2]{\texttt{\frenchspacing\external@render{CONSTPRE:#1@@@#2}}}
\DeclareRobustCommand\isaclass[1]{\texttt{\frenchspacing\external@render{CLASS:#1}}}
\DeclareRobustCommand\isaterm[1]{\texttt{\frenchspacing\external@render{TERM:#1}}}
\DeclareRobustCommand\isatermpre[2]{\texttt{\frenchspacing\external@render{TERMPRE:#1@@@#2}}}
\DeclareRobustCommand\isaprop[1]{\texttt{\frenchspacing\external@render{PROP:#1}}}
\DeclareRobustCommand\isaproppre[2]{\texttt{\frenchspacing\external@render{PROPPRE:#1@@@#2}}}
\DeclareRobustCommand\isatyppre[2]{\texttt{\frenchspacing\external@render{TYPPRE:#1@@@#2}}}
\DeclareRobustCommand\isatyp[1]{\texttt{\frenchspacing\external@render{TYP:#1}}}
\DeclareRobustCommand\isatop[1]{\texttt{\frenchspacing\external@render{TOPLEVEL:@@@#1}}}
\DeclareRobustCommand\isatoppre[2]{\texttt{\frenchspacing\external@render{TOPLEVEL:#1@@@#2}}}
\DeclareRobustCommand\isaabbrev[1]{\texttt{\frenchspacing\external@render{ABBREV:#1}}}
%\DeclareRobustCommand\isalemma[1]{\texttt{\smaller\frenchspacing\external@render{LEMMA:#1}}}
\DeclareRobustCommand\isalemma[1]{\texttt{\frenchspacing\external@render{LEMMA:#1}}}
\DeclareRobustCommand\isalemmapre[2]{\texttt{\frenchspacing\external@render{LEMMAPRE:#1@@@#2}}}
\DeclareRobustCommand\isalocale[1]{\texttt{\frenchspacing\external@render{LOCALE:#1}}}
\DeclareRobustCommand\isathy[2][Complex_Bounded_Operators]{\texttt{\frenchspacing\external@render{THY:#1@@@#2}}}
\DeclareRobustCommand\isasession[1]{\texttt{\frenchspacing\external@render{SESSION:#1}}}
\DeclareRobustCommand\isaattrib[1]{\texttt{\frenchspacing\external@render{ATTRIB:#1}}}
\DeclareRobustCommand\isabundle[1]{\texttt{\frenchspacing\external@render{BUNDLE:#1}}}
\newcommand\isathylong[2]{\texttt{\isasession{#1}.\isathy[{#1}]{#2}}}

\DeclareRobustCommand\isabelletop@env[2]{%
  \begin{quote}%
    \def\externalrendernewline{\\\strut}%
    \def\externalrenderspace{\space}
    \texttt{\frenchspacing\external@render{TOPLEVEL-STRIP-PRE:#1@@@#2}}%
  \end{quote}}

\newenvironment{isabelletoppre}[1]{\catcode`\^^M=12\catcode`\ =12 \def\temp@a{\isabelletop@env{#1}}\Collect@Body\temp@a}{}
\newenvironment{isabelletop}{\catcode`\^^M=12\catcode`\ =12 \def\temp@a{\isabelletop@env{}}\Collect@Body\temp@a}{}

%\def\external@render@TOPLEVEL{TOPLEVEL:}
%\NewEnviron{isabelletop}{\begin{quote}\texttt{\frenchspacing\expandafter\expandafter\expandafter\external@render\expandafter\expandafter\expandafter{\expandafter\external@render@TOPLEVEL\BODY}}\end{quote}}

\newcommand\idxconst[2][]{\index{#2@\isaconst{#2} (constant)\ifx\@nil#1\@nil\else!#1\fi}}
\newcommand\idxtyp[2][]{\index{#2@\isatyp{#2} (type)\ifx\@nil#1\@nil\else!#1\fi}}
\newcommand\idxsession[1]{\index{#1@\isasession{#1} (session)}}
\newcommand\idxlemma[1]{\index{#1@\isalemma{#1} (lemma)}}
\newcommand\idxlocale[1]{\index{#1@\isalocale{#1} (locale)}}
\newcommand\idxclass[2][]{\index{#2@\isaclass{#2} (type class)\ifx\@nil#1\@nil\else!#1\fi}}
\newcommand\idxabbrev[1]{\index{#1@\isaabbrev{#1} (abbreviation)}}
\newcommand\idxbundle[1]{\index{#1@\isabundle{#1} (bundle)}}
\newcommand\idxthy[2][Complex_Bounded_Operators]{\index{#2@\isathy[{#1}]{#2} (theory in \isasession{#1})}}

%\newcommand\isalemmaidx[1]{\isalemma{#1}\idxlemma{#1}}
\newcommand\isaconstidx[2][]{\isaconst{#2}\idxconst[{#1}]{#2}}
\newcommand\isaabbrevidx[2][]{\isaabbrev{#2}\idxabbrev{#2}}
\newcommand\isalocaleidx[1]{\isalocale{#1}\idxlocale{#1}}
\newcommand\isatypidx[2][]{\isatyp{#2}\idxtyp[{#1}]{#2}}
\newcommand\isasessionidx[1]{\isasession{#1}\idxsession{#1}}
\newcommand\isathyidx[2][Complex_Bounded_Operators]{\isathy[{#1}]{#2}\idxthy[{#1}]{#2}}
\newcommand\isaclassidx[2][]{\isaclass{#2}\idxclass[{#1}]{#2}}
\newcommand\isalemmafn[1]{\idxlemma{#1}\footnote{\,\lemmatriangle\,\isalemma{#1}}}
\newcommand\fnsep{\textsuperscript,}


% To make hyperlinked references to footnotes possible with bigfoot footnotes
\patchcmd\FN@fnotecommon\stepcounter\refstepcounter{}\BLABLAerror

\newcommand\pagelabel[1]{\phantomsection\label{#1}}


\newcommand\calH{\mathcal H}

\declare{macro=\lemmatriangle, code={\raisebox{.2ex}{$\scriptstyle\triangleright$}},
  placeholder=\lemmatriangle\,\texttt{lemma\_name},
  description={Reference to the name of a lemma in the Isabelle theories}}

\declare{macro=\ket, argspec=[1], code={\parenthesis\lvert\rangle{#1}},
  placeholder={\ket b},
  description={Basis vector in Hilbert space \texttt{'a ell2}}}

\declare{macro=\bra, argspec=[1], code={\parenthesis\langle\rvert{#1}},
  placeholder={\bra b},
  description={Adjoint of $\bra b$}}

\declare{macro=\setC, code=\mathbb C,
  description={Complex numbers}}

\declare{macro=\setN, code=\mathbb N,
  description={Natural numbers}}

\declare{macro=\abs, argspec=[1], code={\parenthesis\lvert\rvert{#1}},
  placeholder=\abs x, description={Absolute value of $x$}}

\declare{macro=\norm, argspec=[1], code={\parenthesis\lVert\rVert{#1}},
  placeholder=\norm x, description={Norm of vector $x$, \isaconst{norm}}}

\declare{macro=\adj, argspec=[1], code={#1^*}, nopage=true,
  placeholder=\adj A,
  description={Adjoint / conjugate transpose}}

\declare{macro=\cinner, code=\mathop{\isaterm{[*x*]∙⇩C[*y*]}},
  placeholder=\isaterm{ψ ∙⇩C φ},
  description={Inner product, notation for \isaconst{cinner}}}

\declare{macro=\cblinfunA, code={\isatyp{[*'a*]⇒⇩C⇩L[*'b*]}},
  placeholder=\isatyp{'a ⇒⇩C⇩L 'b},
  description={Type of bounded operators, notation for~\isatyp{cblinfun}}}

\declare{macro=\cbapplyISA, code={\isaterm{[* f *]*⇩V[* x *]}},
  placeholder=\isaterm{f *⇩V x},
  description={Applying bounded operator \isaterm{f} to vector \isaterm{x}; notation for \isaconst{cblinfun_apply}}}

\declare{macro=\oCL, code={\isaterm{[*A*]o⇩C⇩L[*B*]}},
  placeholder=\isaterm{A o⇩C⇩L B},
  description={Composition of bounded operators, notation for~\isaconst{cblinfun_compose}}}

\declare{macro=\cblinfunImage, code={\isaterm{[*A*]*⇩S[*S*]}},
  placeholder=\isaterm{A *⇩S S},
  description={Image of subspace under a bounded operator, notation for~\isaconst{cblinfun_image}}}

\declare{macro=\scaleC, code={\isaterm{[*c*]*⇩C[*x*]}},
  placeholder=\isaterm{c *⇩C ψ},
  description={Scalar multiplication, notation for \isaconst{scaleC}}}

\declare{macro=\closedSum, code={\isaterm{[*A*]+⇩M[*B*]}},
  placeholder=\isaterm{A +⇩M B},
  description={Closed sum of sets, notation for \isaconst{closed_sum}}}

\declare{macro=\adjISA, code={\isaterm{[*A*]*}},
  placeholder=\isaterm{A*},
  description={Adjoint of \isaterm{A}}}

\declare{macro=\topISA, code=\top,
  description={Top element of a lattice (\isaconst{top}), e.g. the whole space}}

\declare{macro=\Sup, code=\sqcup,
  placeholder=x \sqcup y,
  description={Binary supremum \isaconst{sup}}}

\declare{macro=\Inf, code=\sqcap,
  placeholder=x \sqcap y,
  description={Binary infimum \isaconst{inf}}}

\declare{macro=\elltwo, code=\ell_2,
  placeholder=\ell_2(X),
  description={Square summable functions $X\to\setC$, Isabelle type \isatyp{'x ell2}}}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "bounded-operators"
%%% End:

